Characterizing Co-located Datacenter Workloads: An Alibaba Case Study

Warehouse-scale cloud datacenters co-locate workloads with different and often complementary characteristics for improved resource utilization. To better understand the challenges in managing such intricate, heterogeneous workloads while providing quality-assured resource orchestration and user experience, we analyze Alibaba's co-located workload trace, the first publicly available dataset with precise information about the category of each job. Two types of workload---long-running, user-facing, containerized production jobs, and transient, highly dynamic, non-containerized, and non-production batch jobs---are running on a shared cluster of 1313 machines. Our multifaceted analysis reveals insights that we believe are useful for system designers and IT practitioners working on cluster management systems.

==> Makefile <==
.SUFFIXES: .tex .dvi .ps .fig .eps .gnu .c
#PDF = ps2pdf -dPDFSETTINGS=/printer -dMaxSubsetPct=100 -dCompatibilityLevel=1.4 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=letter -dUseCIEColor
PDF = ps2pdf14 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true \
	       -dSubsetFonts=true -dMaxSubsetPct=100

TARGET=paper
DOBIB=yes
VIEWER=evince

HOST=$(shell hostname)

.PHONY: $(TARGET)

all:	display


display: $(TARGET)
	#dvips -Ppdf -G0 $(TARGET).dvi -o $(TARGET).ps
	pdflatex $(TARGET).tex
	#$(PDF) $(TARGET).ps
#ifeq ($(USER),  butta)
#	evince paper.pdf
#endif
#ifeq ($(HOST),  tddg)
#	open paper.pdf
#else
#	evince paper.pdf
#endif

#display: $(TARGET)
#	dvips -Ppdf -G0 $(TARGET).dvi -o $(TARGET).ps
#	$(PDF) $(TARGET).ps
#	$(VIEWER) $(TARGET).pdf

$(TARGET): $(TARGET).tex
#	latex $(TARGET)
	pdflatex $(TARGET)
ifeq ($(DOBIB),yes)
	bibtex $(TARGET)
	pdflatex $(TARGET)
	pdflatex $(TARGET)
endif

clean:
	$(RM) $(TARGET).ps $(TARGET).pdf $(TARGET).log $(TARGET).out $(TARGET).aux $(TARGET).dvi $(TARGET).tex.flc
	$(RM) $(TARGET).bbl $(TARGET).blg
	$(RM) *.kill kill*

purge:	clean
	$(RM) *~

nums:
	cd numbers;gnuplot plotGraph

spell:
	cat $(TF) | awk '{ if (index($$0,"%")!=1) print $$0}' |  spell 
#	detex $(TF) |  spell 

strip: $(TARGET)
	mkdir -p stripped/source
	for a in `ls --color=auto *.tex`; do cat $$a | awk '{ if (index($$0,"%")!=1) print $$0}' >stripped/source/$$a; done
	(cd stripped/source; \
	cat paper.tex | awk '{if (match($$0, "\\input")==0) print $$0; else {sub( /}/, ".tex", $$xx); sub(/\\input{/, "", $$xx);  system("cat " $$xx);}}'  > step1; \
	rm *.tex; \
	mv step1 paper.tex; \
	cp ../../paper.bbl .; \
	cd ../..)
	pwd
	(cd stripped/source; files=`ls --color=auto *.eps`; \
	cd ../..; cp $$files stripped/source/; )
	(for dirs in figure plot2 plot3; \
	do cd stripped/source/$$dirs; \
	files=`ls --color=auto *.eps`; \
	cd ../../../$$dirs; \
	cp $$files ../stripped/source/$$dirs; \
	cd ..; \
	done )



==> casestudy.tex <==
\vspace{-5pt}
\section{Case Study}
\label{sec:case}


%\begin{figure}[t]
%\begin{center}
%\subfigure[CPU usage.] {
%\includegraphics[width=.235\textwidth]{plots/cpu_b_lr.pdf}
%%\vspace{-10pt}
%\label{fig:col_cpu}
%}
%\hspace{-1.4em}
%\subfigure[Memory usage.] {
%\includegraphics[width=.235\textwidth]{plots/mem_b_lr.pdf}
%%\vspace{-10pt}
%\label{fig:col_mem}
%}
%\vspace{-15pt}
%\caption{{\small
%Box-and-whisker plots showing CPU and memory usage distributions.
%{\small\texttt{Batch only}}: the machine region hosting batch jobs only;
%{\small\texttt{Batch co-located}}: batch jobs' resource usage in region  
%hosting both batch and long-running applications (LRA);
%{\small\texttt{LRA co-located}}: LRA's resource usage in region hosting both.
%}}
%\label{fig:col_usage}
%\end{center}
%\vspace{-15pt}
%\end{figure}



==> discussion.tex <==
%\vspace{-10pt}
\section{Discussion Points}
\vspace{-10pt}

%\Comment{yuec: more content added here...exceeding the half page limit...switched to small fonts...}

While a lot of research has looked at the technical aspects of
building clouds, their impact and their use by the tenants, we
believe the current cloud pricing mechanism (especially for storage
services) is vague and lacks transparency.  In this work, we have
attempted to reconcile the economic principles of demand and supply with
the technical aspects of storage tiering through dynamic pricing to
showcase the benefits for both the cloud provider as well as the
tenants.

We believe that our paper will lead to discussion on the following
points of interest:
(1)~The need for revisiting pricing strategies in established hybrid
storage deployments and practices. Since storage tiering is a well-studied area, we
believe that the paper will lead to hot discussion on how the
paradigm shift is happening, and why the extant approaches and ideas need to be revisited.
A particular point of interest in the context of tiering is that the
objectives of different players are often times in conflict.
%(b)
%The finer details of cloud-controlled and tenant-demand based dynamic
%pricing for cloud services and storage in particular.
(2)~Issues such as how useful can our pricing ``knob'' be for the cloud
provider to shape tenant behavior to suit the provider requirements, and at
what granularity should the proposed price variations be implemented, are
part of our future work and would make for a productive discussion. 
(3)~The role of flash and other emerging technologies in cloud-based
object stores.

An unexplored issue is tenant behavior modeling. Our preliminary
results assume a smart tenant using models described in
\cref{sec:design}. However, in reality, tenants can have very
different behaviors and utility functions. Furthermore, we have not
looked at multi-tenancy in detail. For instance, a ``naive'' or ``rogue'' tenant that
performs a lot of SSD writes without considering their utility can cause the
cloud to increase the price of SSDs, thus affecting the utility of other
well-behaved tenants. 
%\tobeadded{
%As the cloud and tenants can only make ``myopic'' decisions based on partial information,
%%based on which they make ``myopic'' decisions. 
%we also need to evaluate the goodness of our predictors of both the
%tenant's future demand and the cloud's future pricing behavior in the
%presence of this incomplete information, especially in a
%multi-tenancy environment.
%}
%In order to tackle such issues, we are considering introducing the
%notion of tenant specific QoS 
Another open aspect of our current work is investigating the game
theoretic results of our model. These include the
behavior of provider's profit and the tenant's utility when the
system reaches equilibrium and the comparison of these objectives
under Nash and Stackelberg equilibria.
%
%From a systems development point of view, the biggest challenge to
%determine is whether a prototype (e.g., using OpenStack Swift) would
%yield similar benefits as shown through preliminary simulation
%results. If in prototyping the bottlenecks turn out to be something
%other than device performance (e.g., software overheads, metadata
%issues, network bandwidth problems, etc.), then the merit of tiering
%vs. the complexity it introduces ``might'' reduce diminishing the value
%of the work. 

Furthermore, prices of SSDs are falling. Even though the gap
between HDD and SSD prices is still wide today, in the future with
increase in NAND flash production, improvement in flash yields,
lithographic improvements such as 3D stacking, etc., can reduce the
price difference, 
%decreasing the value of tiering and 
resulting in SSDs becoming the de facto storage medium in cloud
environments.  
%SSD lifetime issues can also be solved through software
%techniques (the improved density through 3-bit MLC NAND seems to have
%taken a toll on SSD endurance but software techniques such as
%stronger ECC hold promise for maintaining the SSD reliability). 
%Moreover, lower SSD prices can affect the margins for the cloud
%providers reducing the profit for the cloud. 
From the tenant side, while researchers have shown the merit of using
SSDs (e.g., in interactive HBase
workloads~\cite{hbase_analysis_fast14}), their use in batch-oriented
analytics workloads is just starting. Indeed, in another research
work~\cite{cast_hpdc15}, we have shown through real experiments on
Google Cloud that SSDs can provide great benefits especially
when considering heterogeneity in cloud storage services, 
%e.g., block SSDs and ephemeral SSDs etc., 
enforcing our belief that our future hybrid object store prototyping
efforts will yield desirable win--win solutions.

%the merit of tiering vs. the complexity it introduces need to
%evaluated in detail.

%   Finally, we look forward to 
%   receive positive feedback (what aspects the workshop
%   participants like about our work), as well as constructive criticism
%   (what areas we have missed, overlooked or need to investigate in more
%   detail) on the various aspects described above.


==> related.tex <==
%\vspace{-12pt}
\section{Related Work}
\label{sec:related}

